Linear Shift-Register Synthesis for Multiple Sequences of Varying Length

The problem of finding the shortest linear shift-register capable of generating t finite length sequences over some field F is considered. A similar problem was already addressed by Feng and Tzeng. They presented an iterative algorithm for solving this multi-sequence shift-register synthesis problem, which can be considered as generalization of the well known Berlekamp-Massey algorithm. The Feng-Tzeng algorithm works indeed, if all t sequences have the same length. This paper focuses on multi-sequence shift-register synthesis for generating sequences of varying length. It is exposed, that the Feng-Tzeng algorithm does not always give the correct solution in this case. A modified algorithm is proposed and formally proved, which overcomes this problem.

==> defs.tex <==
\DeclareMathAlphabet{\mathbcal}{OMS}{cmsy}{b}{n}

\DeclareMathOperator{\de2}{d^2_{\mathcal{E}}}
\DeclareMathOperator{\depth}{depth}
\DeclareMathOperator{\wt}{wt}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\neras}{\mathcal{N}}
\DeclareMathOperator{\erfc}{erfc}
\DeclareMathOperator{\sort}{sort}

\newcommand{\eras}{\ensuremath{\varepsilon}}

\newcommand{\eproj}[2]{\ensuremath{P_{\neras({#1})}\left[{#2}\right]}}

\newcommand{\set}[1]{\ensuremath{#1}}
\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\vect}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\mat}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\submatr}[3]{\ensuremath{left.\boldsymbol{#1}\right|_{#2}^{#3}}}
%\newcommand{\srt}[1]{\ensuremath{{#1}\!\raisebox{1pt}{$\downharpoonright$}}}
\newcommand{\srt}[1]{\ensuremath{\check{#1}}}

\newcommand{\Cu}[1]{\ensuremath{\sigma^{\langle{#1}\rangle}}}
\newcommand{\Ct}{\ensuremath{\Sigma}}

\newcommand{\card}[1]{\ensuremath{\left|{#1}\right|}}
\newcommand{\code}{\ensuremath{\mathcal{C}}}
\newcommand{\codeo}{\ensuremath{\mathcal{A}}}
\newcommand{\codei}{\ensuremath{\mathcal{B}}}
\newcommand{\rscode}{\ensuremath{\mathcal{C}_{\text{RS}}}}
\newcommand{\BCH}{\ensuremath{\text{BCH}}}
\newcommand{\RS}[1]{\ensuremath{\mathcal{RS}\left({#1}\right)}}
\newcommand{\Golay}[1]{\ensuremath{\mathcal{G}\left({#1}\right)}}
\newcommand{\IRS}[1]{\ensuremath{\mathcal{IRS}\left({#1}\right)}}
\newcommand{\F}[1]{\ensuremath{\mathbb{F}}_{#1}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\CE}{\ensuremath{\mathcal{E}}}
\newcommand{\FF}[2]{\ensuremath{\mathbb{F}}_{#1}^{#2}}
\newcommand{\GF}[1]{\ensuremath{\text{GF}}\left({#1}\right)}

\newcommand{\Seq}{\ensuremath{\mathcal{S}}}
\newcommand{\XSeq}{\ensuremath{\mathcal{X}}}

\newcommand{\nset}{\ensuremath{\mathcal{N}}}
\newcommand{\mset}{\ensuremath{\mathcal{M}}}

\newcommand{\FT}[1]{\ensuremath{\mathfrak{F}\left({#1}\right)}}
\newcommand{\IFT}[1]{\ensuremath{\mathfrak{F}^{-1}\left({#1}\right)}}

\newcommand{\alg}[1]{\textsf{{#1}}}

\newcommand{\svform}[1]%
{\begin{sideways}\footnotesize\ensuremath{{#1}\;}\end{sideways}}

% trellis stuff
\newcommand{\edg}{\ensuremath{\varepsilon}}
\newcommand{\nod}{\ensuremath{\nu}}
\newcommand{\lbl}{\ensuremath{\lambda}}
\newcommand{\ilbl}{\ensuremath{\lambda^i}}
\newcommand{\edgset}{\ensuremath{\mathcal E}}
\newcommand{\nodset}{\ensuremath{\mathcal V}}
\newcommand{\lblset}{\ensuremath{\mathcal L}}
\newcommand{\edgcard}{\ensuremath{|\mathcal E|}}
\newcommand{\nodcard}{\ensuremath{|\mathcal V|}}
\newcommand{\snode}[1]{\ensuremath{\alpha\left({#1}\right)}}
\newcommand{\enode}[1]{\ensuremath{\omega\left({#1}\right)}}
\newcommand{\epath}{\ensuremath{\boldsymbol{\pmb\varepsilon}}}
\newcommand{\tepath}{\ensuremath{\boldsymbol{\widetilde{\pmb\varepsilon}}}}
\newcommand{\pathset}[1]{\ensuremath{{\mathbcal E}\left({#1}\right)}}
\newcommand{\eseg}[2]{\ensuremath{\left.{\epath}\right|_{#1}^{#2}}}
\newcommand{\esegi}[3]{\ensuremath{\left.{\epath}_{#1}\right|_{#2}^{#3}}}
\newcommand{\ccseg}{\ensuremath{\parallel}}
\newcommand{\segset}{\ensuremath{\mathcal D}}
\newcommand{\tset}{\ensuremath{\mathcal S}}
\newcommand{\tail}[1]{\ensuremath{{\mathcal T}\left({#1}\right)}}
\newcommand{\head}[1]{\ensuremath{{\mathcal H}\left({#1}\right)}}
\newcommand{\tailp}[1]{\ensuremath{{\mathcal T}^\prime\left({#1}\right)}}
\newcommand{\inset}[1]{\ensuremath{{\mathcal I}\left({#1}\right)}}
\newcommand{\insubset}[1]{\ensuremath{{\mathcal J}\left({#1}\right)}}
\newcommand{\insubsetp}[1]{\ensuremath{{\mathcal J}^\prime\left({#1}\right)}}
\newcommand{\outset}[1]{\ensuremath{{\mathcal O}\left({#1}\right)}}
\newcommand{\nodmetset}[1]{\ensuremath{{\mathcal M}\left({#1}\right)}}

\newcommand{\algcomment}[1]{\textsf{\footnotesize/$\ast$\ {#1}$\ \ast$/}}

\makeatletter
\newcommand{\ncirc}[1]{%
        \leavevmode\hbox{\setbox0=\hbox{\ensuremath{#1}}\relax
        \dimen0=\the\wd0\dimen1=\the\ht0
        \ifdim\dimen0>\dimen1\dimen2=\dimen0\else\dimen2=\dimen1\fi
        \divide\dimen0 by 2\divide\dimen1 by 2\advance\dimen2 by 5pt
        \put(\strip@pt\dimen0, \strip@pt\dimen1){\circle{\strip@pt\dimen2}}
        \box0}%
}
\newcommand{\mcirc}[1]{%
        \leavevmode\hbox{\setbox0=\hbox{\scriptsize\ensuremath{#1}}\relax
        \dimen0=\the\wd0\dimen1=\the\ht0
        \ifdim\dimen0>\dimen1\dimen2=\dimen0\else\dimen2=\dimen1\fi
        \divide\dimen0 by 2\advance\dimen0 by -0.4pt
        \divide\dimen1 by 2\advance\dimen1 by -1pt\advance\dimen2 by 1.80pt
        \put(\strip@pt\dimen0, \strip@pt\dimen1){\circle{\strip@pt\dimen2}}
        \box0}%
}
\newcommand{\nbox}[1]{\setlength{\fboxsep}{1.0pt}\fbox{\ensuremath{{#1}}}}
\makeatother

\newcommand{\tmgbox}[1]{\psboxit{box .9 setgray fill}
                     {\setlength{\fboxsep}{1pt}%
                      \spbox{\scriptsize \ensuremath{#1}}}}

